The role of the elaphrocentre in void galaxy formation

Voids may affect galaxy formation via weakening mass infall or increasing disk sizes, which could potentially play a role in the formation of giant low surface brightness galaxies (LSBGs). If a dark matter halo forms at the potential hill corresponding to a void of the cosmic web, which we denote the 'elaphrocentre' in contrast to a barycentre, then the elaphrocentre should weaken the infall rate to the halo when compared to infall rates towards barycentres. We investigate this hypothesis numerically. We present a complete software pipeline to simulate galaxy formation, starting from a power spectrum of initial perturbations and an N-body simulation through to merger-history-tree based mass infall histories. The pipeline is built from well-established, free-licensed cosmological software packages, and aims at highly portable long-term reproducibility. We find that the elaphrocentric accelerations tending to oppose mass infall are modest. We do not find evidence of location in a void or elaphrocentric position weakening mass infall towards a galaxy. However, we find indirect evidence of voids influencing galaxy formation: while void galaxies are of lower mass compared to galaxies in high density environments, their spin parameters are typically higher. For a fixed mass, the implied disk scale length would be greater. Tangential accelerations in voids are found to be high and might significantly contribute to the higher spin parameters. We find significantly later formation epochs for void galaxies; this should give lower matter densities and may imply lower surface densities of disk galaxies. Thus, void galaxies have higher spin parameters and later formation epochs; both are factors that may increase the probability of forming LSBGs in voids.

==> Makefile <==
paper.pdf: paper-full.tex
	latex paper-full && latex paper-full && latex paper-full \n	&&dvips paper-full -o paper-tmp.eps \n	&&ps2pdf paper-tmp.eps \n	&&mv -v paper.pdf elaphrocentre.pdf

.PHONY: clean
clean:
	rm -f *.aux *.auxlock *.bbl *.bcf
	rm -f *.blg *.log *.out *.run.xml

